DrAttack: Prompt Decomposition and Reconstruction Makes Powerful LLM Jailbreakers

The safety alignment of Large Language Models (LLMs) is vulnerable to both manual and automated jailbreak attacks, which adversarially trigger LLMs to output harmful content. However, current methods for jailbreaking LLMs, which nest entire harmful prompts, are not effective at concealing malicious intent and can be easily identified and rejected by well-aligned LLMs. This paper discovers that decomposing a malicious prompt into separated sub-prompts can effectively obscure its underlying malicious intent by presenting it in a fragmented, less detectable form, thereby addressing these limitations. We introduce an automatic prompt \textbf{D}ecomposition and \textbf{R}econstruction framework for jailbreak \textbf{Attack} (DrAttack). DrAttack includes three key components: (a) `Decomposition' of the original prompt into sub-prompts, (b) `Reconstruction' of these sub-prompts implicitly by in-context learning with semantically similar but harmless reassembling demo, and (c) a `Synonym Search' of sub-prompts, aiming to find sub-prompts' synonyms that maintain the original intent while jailbreaking LLMs. An extensive empirical study across multiple open-source and closed-source LLMs demonstrates that, with a significantly reduced number of queries, DrAttack obtains a substantial gain of success rate over prior SOTA prompt-only attackers. Notably, the success rate of 78.0\% on GPT-4 with merely 15 queries surpassed previous art by 33.1\%. The project is available at https://github.com/xirui-li/DrAttack.

==> 7_impact.tex <==
\section*{Broader Impact}

This research presents DrAttack, a novel technique for jailbreaking LLMs through prompt decomposition and reconstruction. While the primary focus is on understanding and exposing vulnerabilities within LLMs, it is crucial to consider the dual-use nature of such findings. This work demonstrates the ease with which LLMs can be manipulated, raising essential questions about their security in real-world applications. We intend to stimulate the development of more robust defenses against such vulnerabilities, thereby contributing to LLMs' overall resilience and reliability.

However, we acknowledge the potential for misuse of these techniques. The methods demonstrated could be leveraged by malicious actors to bypass safeguards in LLMs, leading to unethical or harmful applications. 
Despite the potential risk, the technique is simple to implement and may be ultimately discovered by any malicious attackers, 
so disclosing this technique is essential for developing defensive mechanisms to improve the safety of current LLM systems. 
By highlighting these vulnerabilities, we aim to foster a community-wide effort towards more secure and responsible AI development.
